Fair Active Learning

Machine learning (ML) is increasingly being used in high-stakes applications impacting society. Therefore, it is of critical importance that ML models do not propagate discrimination. Collecting accurate labeled data in societal applications is challenging and costly. Active learning is a promising approach to build an accurate classifier by interactively querying an oracle within a labeling budget. We design algorithms for fair active learning that carefully selects data points to be labeled so as to balance model accuracy and fairness. We demonstrate the effectiveness and efficiency of our proposed algorithms over widely used benchmark datasets using demographic parity and equalized odds notions of fairness.

==> Archive/fbc.tex <==
% \vspace{-5mm}
\section{Efficient FAL by Covariance}\label{sec:fbc}
% \vspace{-3mm}
%Labeling is the major cost in active learning settings.
%In societal applications, the labeling cost often dominates the computation cost.
In this section we propose a computationally efficient alternative for FAL.
% hence the running time of the sampling algorithm is usually not a major concern.
The fair active learning algorithm proposed in \S~\ref{sec:framework} requires to compute the expected fairness for every instance in the unlabeled pool $\mathcal{U}$ before deciding on the next sample point to label by building $K$ models, one for each possible label.
%For every unlabeled instance, computing the expected fairness requires building $K$ models for each possible label.
%This process is inefficient:
Suppose the time to build a model is $T$; for the labeling budget $B$ and a constant value $K$, the algorithm requires the time complexity of $O(B \cdot T \cdot |\mathcal{U}|)$ to build the models.
%One idea to make the process more efficient is to reduce the size of the unlabeled pool by selecting an unbiased sample set from $\mathcal{U}$.
%Another idea to reuse the current model by updating it based on the new sample. This has been extensively studied, specifically for SVM, in the context of streaming and online learning~\cite{gepperth2016incremental}.
%For gradient-descend based learning methods also, one can use the current model parameters as the starting point.
% Most of the existing work, however, provide approximations that would add an error to the computation of expected fairness improvement.

% Both of the above approaches are perfectly valid and we recall once again that the major cost in AL is labeling.
For the special case of  generalized linear models, we design an efficient algorithm 
that has the \emph{same} asymptotic time complexity as traditional active learning.
%As an efficient alternative for fair active learning, in this section we propose an alternative method for achieving fairness for generalized linear models
We achieve this by avoiding the retraining of models to calculate the expected fairness of unlabeled samples.
%
Consider a generalized linear model in form of $\hat{y}=\theta^\top X$.\footnote{The decision boundary of the classifier is viewed as a threshold value on $\hat{y}$ that separate different classes, using, for example, a sign function.} %\hadis{if y hat is a classifier it needs a sign or sigmoid function.}
Recall that under model independence (demographic parity) the covariance between the model and a sensitive attribute $S$ is zero.
We make a key observation in Lemma~\ref{th:cov} that shows this covariance, $cov(S,\hat{y})$, {\em only depends on $cov(S,X)$ and $\theta$}.
% In other words, the underlying covariance $cov(S,X)$ can cause model unfairness.

\begin{lemma}\label{th:cov}
For a generalized linear model in form of $\hat{y}=\theta^\top X$,
% Under the Assumption 1.
$cov(S,\hat{y})=\theta^\top cov(S,X)$.
% \footnote{The proof of Lemma~\ref{th:cov} can be found in the \techrep{Appendix}\submit{supplementary material}.}
\end{lemma}
\begin{proof}
\begin{align*}
    cov(S,\hat{y})&=E[S\, \hat{y}] - E[S]E[\hat{y}]\\
    E[S]E[\hat{y}] &= \mu_S E\big[\sum\theta_ix_i\big] = \mu_S \sum\theta_i\mu_{x_i}\\ &=\theta_1\mu_S\mu_{x_1}+\theta_2\mu_S\mu_{x_2}+\cdots+\theta_d\mu_S\mu_{x_d}\\
    E[S\hat{y}]&= E\big[S\,\sum\theta_ix_i\big] = E\big[\sum S\, \theta_ix_i\big] \\ 
    & = E\big[S\,\theta_1x_1+S\,\theta_2x_2+\cdots+ S\,\theta_d x_d \big]\\
    &=E\big[S\,\theta_1x_1\big]+E\big[S\,\theta_2x_2\big]+\cdots+ E\big[S\,\theta_d x_d \big]\\
    &=\theta_1E\big[S\,x_1\big]+\cdots+ \theta_d E\big[S\, x_d \big]
\end{align*}

\begin{align*}
    \Rightarrow cov(S,\hat{y})&=
    \theta_1E\big[S\,x_1\big]+\cdots+ \theta_d E\big[S\, x_d \big] \\
    &~~~~- (\theta_1\mu_S\mu_{x_1}+\cdots+\theta_d\mu_S\mu_{x_d})\\
    &=\theta_1(E\big[S\,x_1\big] - \mu_S\mu_{x_1})+\cdots+
    \theta_d(E\big[S\,x_d\big] - \mu_S\mu_{x_d}) \\
    &= \sum\limits_{i=1}^d \theta_i cov(S,x_i) = \theta^\top cov(S,X)
\end{align*}
\end{proof}
%Proof moved to supplementary.tex
%\begin{proof}
%% $cov(S,\hat{y})$ can be computed as $\theta^\top cov(S,X)$:
%\begin{align*}
%    cov(S,\hat{y})&=E[S\, \hat{y}] - E[S]E[\hat{y}]\\
%    E[S]E[\hat{y}] &= \mu_S E\big[\sum\theta_ix_i\big] = \mu_S \sum\theta_i\mu_{x_i} =\theta_1\mu_S\mu_{x_1}+\theta_2\mu_S\mu_{x_2}+\cdots+\theta_d\mu_S\mu_{x_d}\\
%    E[S\hat{y}]&= E\big[S\,\sum\theta_ix_i\big] = E\big[\sum S\, \theta_ix_i\big] =E\big[S\,\theta_1x_1+S\,\theta_2x_2+\cdots+ S\,\theta_d x_d \big]\\
%    &=E\big[S\,\theta_1x_1\big]+E\big[S\,\theta_2x_2\big]+\cdots+ E\big[S\,\theta_d x_d \big]=\theta_1E\big[S\,x_1\big]+\cdots+ \theta_d E\big[S\, x_d \big]
%\end{align*}

%\begin{align}
%    \nonumber \Rightarrow& cov(S,\hat{y})=
%    \theta_1E\big[S\,x_1\big]+\theta_2E\big[S\,x_2\big]+\cdots+ \theta_d E\big[S\, x_d \big] - (\theta_1\mu_S\mu_{x_1}+\cdots+\theta_d\mu_S\mu_{x_d})\\
%    \nonumber =&\theta_1(E\big[S\,x_1\big] - \mu_S\mu_{x_1})+\cdots+
%    \theta_d(E\big[S\,x_d\big] - \mu_S\mu_{x_d}) = \sum\limits_{i=1}^d \theta_i cov(S,x_i) = \theta^\top cov(S,X)
%\end{align}
%\end{proof}


According to Lemma~\ref{th:cov}, the covariance of the model with the sensitive attribute (that results in unfairness) depends only on the weight vector $\theta$ and the underlying covariance of features $X$ with $S$.
To make the model fairer, we need to ensure that the model does not assign high weights to the problematic features (the features with high covariance with $S$).
This observation allows us to indirectly optimize for fairness through covariance instead of computing expected fairness.


% for a specific tuple and a feature
Consider a feature $x_i$ that is highly correlated with the sensitive attribute (i.e., $cov(x_i,S)$ is high) and also has a high weight $\theta_i$ in the current model. Our objective is to reduce the weight assigned to such features.
The reason the model has assigned a large weight to $x_i$ is that {\em $x_i$ is highly predictive of $y$ in $\mathcal{L}$}. In other words, $x_i$ is a good signal for predicting $y$ according to $\mathcal{L}$.
% The high covariance between $x_i$ and $y$ in $\mathcal{L}$ has made it a valuable signal for the model to predicting $y$.
Therefore, in order to reduce the weight $\theta_i$, we need to reduce $cov_{\mathcal{L}}(x_i,y)$ in the labeled pool $\mathcal{L}$ to make it less predictive of $y$ in $\mathcal{L}$.
%
Now, consider a point $P_j = \langle X^{(j)}, S^{(j)} \rangle\in \mathcal{U}$ and its value $X^{(j)}_i$ on feature $x_i$.
Depending on $X^{(j)}_i$ and its label $y^j$ (after labeling), the point $P_j$ can impact $cov(x_i,y)$ in $\mathcal{L}$.
Of course we don't know $y^j$; still, similar to \S~\ref{sec:alg}, we can consider the probability distribution over $Y$ and calculate the expected improvement in covariance.
%treat the covariance improvement as expected value.
Let $cov_i = cov_{\mathcal{L}}(x_i,y)$ be the covariance of $x_i$ and $y$ in $\mathcal{L}$
and $cov_{j,i,k} = cov_{\mathcal{L}\cup\{\langle X^{(j)}, S^{(j)},y^{(j)}=k \rangle\}}(x_i,y)$
the covariance of $x_i$ and $y$ after adding $\langle X^{(j)}, S^{(j)},y^{(j)}=k \rangle$ to $\mathcal{L}$.
The expected covariance improvement for $x_i$ after adding $P_j$ to $\mathcal{L}$ is
%\vspace{-2mm}
\begin{align} \label{eq:efibc}
E\big[cov^{\downarrow}_{j,i} \big]  = \sum_{k=0}^{K-1} (|cov_i| - |cov_{j,i,k}|) \mathbb{P}(y=k|X^{(j)})
\end{align}
Following Lemma~\ref{th:cov} the contribution of the covariance reduction for a feature $x_i$ to fairness is proportional to $\theta_i cov(x_i,S)$.
Subsequently, it is important to reduce $cov_{\mathcal{L}}(x_i,y)$ for the features that are highly correlated with the sensitive attribute and have a high weight $\theta_i$ in the model.
Therefore, the (indirect) fairness improvement by covariance for a point $P_j\in\mathcal{U}$ can be computed as following:
%\vspace{-2mm}
\begin{align}\label{eq:efbc}
    E\big[FbC^{\downarrow}_{j} \big] =
    \sum\limits_{i=1}^d \theta_i cov(S,x_i) E\big[cov^{\downarrow}_{j,i} \big]
\end{align}
Now, it is enough to replace the term for expected fairness improvement $\big(\mathcal{F}(C_{t-1})-\mathcal{F}(C_{t}^i)\big)$ in Equation~\ref{eq:opt} by $E\big[FbC^{\downarrow}_{i} \big]$.
%In \submit{the supplementary material}\techrep{the Appendix}, 



\subsection{Efficiently Computing Covariance of $X$ and $y$ in $\mathcal{L}$}
So far in this section, we proposed the efficient FAL by covariance method that works based on Equation~\ref{eq:efbc}. Considering the number of features $d$ as a constant, we now show how, maintaining the aggregates from the previous steps, $E\big[FbC^{\downarrow}_{j} \big]$ can be computed in {\em constant time}.
Therefore, the time complexity of the fair active learning framework (without considering the labeling cost) drops from $O(B \cdot T \cdot |\mathcal{U}|)$ to $O\big(B \cdot (|\mathcal{U}|+T)\big)$, {\em the same as traditional active learning}.
%In the following we show the details of computing $E\big[FbC^{\downarrow}_{j} \big]$ for every point $P_j\in\mathcal{U}$ in constant time, maintaining the aggregates from the previous steps.

First, we note that $cov(x_i,S)$, the covariance of each feature $x_i$ with $S$, does not depend on $\mathcal{L}$ and can be computed in advance, using the unlabeled samples in $\mathcal{U}$. It is computed once for every feature at the beginning of the process and the same numbers will be used in different iterations. 
The values of $cov_i = cov_{\mathcal{L}}(x_i,y)$ and $cov_{j,i,k} = cov_{\mathcal{L}\cup\{\langle X^{(j)}, S^{(j)},y^{(j)}=k \rangle\}}(x_i,y)$ in Equation~\ref{eq:efibc},
however, depend on the set of labeled data and should get recomputed at different iterations and for different points $P_j\in\mathcal{U}$.
We maintain the following aggregates for efficiently computing these values:
\begin{align*}
    &~ \mathcal{G}_y ~= \sum_{\forall \langle X^{(\ell)},S^{(\ell)},y^{(\ell)}\rangle\in\mathcal{L}} y^{(\ell)}\\
    \forall i\in[1,d]: ~& \mathcal{G}_x[i] = \sum_{\forall \langle X^{(\ell)},S^{(\ell)},y^{(\ell)}\rangle\in\mathcal{L}} X^{(\ell)}_i\\
        \forall i\in[1,d]: ~& \mathcal{G}_z[i] = \sum_{\forall \langle X^{(\ell)},S^{(\ell)},y^{(\ell)}\rangle\in\mathcal{L}} X^{(\ell)}_i y^{(\ell)}
\end{align*}

Note that at every iteration each of the above aggregates can be updated in constant time by adding the corresponding value from the new point to it.
Now, using these aggregates:
$$cov_i = cov_{\mathcal{L}}(x_i,y) = \frac{\mathcal{G}_z[i]}{n} - \frac{\mathcal{G}_x[i]}{n}\times\frac{\mathcal{G}_y}{n}$$
Similarly, for a point $P_j = \langle X^{(j)}, S^{(j)} \rangle\in\mathcal{U}$ and a label $y^{(j)}=k$:
$$cov_{j,i,k} = \frac{\mathcal{G}_z[i] + k X^{(j)}_i}{n+1} - \frac{\mathcal{G}_x[i] + X^{(j)}_i }{n+1}\times\frac{\mathcal{G}_y + k}{n+1}$$


%Moved to supplementary.tex
% how to update the aggregates?
%\subsection{Computing covariance measures\abol{this can go to appendix/tech rep}}
%In the following we show the details of computing Equation~\ref{eq:efbc} for every point $P_j\in\mathcal{U}$ in constant time, maintaining the aggregates from the previous steps.

%First, we note that $cov(x_i,S)$, the covariance of a feature $x_i$ with $S$, does not depend on $\mathcal{L}$ and can be computed using the unlabeled samples in $\mathcal{U}$. It is computed once for every feature at the beginning of the process and the same numbers will be used for different iterations.

%The values of $cov_i$ and $cov_{j,i,k}$ in Equation~\ref{eq:efibc}, however, do depend on the set of labeled data and should get recomputed at different iterations and for different points $P_j\in\mathcal{U}$.
%We maintain the following aggregates for efficiently computing these values:
%\begin{align*}
%    &~ S_y ~= \sum_{\forall \langle X^{(\ell)},S^{(\ell)},y^{(\ell)}\rangle\in\mathcal{L}} y^{(\ell)}\\
%    & \forall i\in[1,d]: ~ S_x[i] = \sum_{\forall \langle X^{(\ell)},S^{(\ell)},y^{(\ell)}\rangle\in\mathcal{L}} X^{(\ell)}_i; ~ S_z[i] = \sum_{\forall \langle X^{(\ell)},S^{(\ell)},y^{(\ell)}\rangle\in\mathcal{L}} X^{(\ell)}_i y^{(\ell)}
%\end{align*}

%Note that at every iteration each of the above aggregates can be updated in constant time by adding the corresponding value from the new point to it.
%Now, using these aggregates:
%$$cov_i = cov_{\mathcal{L}}(x_i,y) = \frac{S_z[i]}{n} - \frac{S_x[i]}{n}\times\frac{S_y}{n}$$
%Similarly, for a point $P_j = \langle X^{(j)}, S^{(j)} \rangle\in\mathcal{U}$ and a label $y^{(j)}=k$:
%$$cov_{j,i,k} = \frac{S_z[i] + k X^{(j)}_i}{n+1} - \frac{S_x[i] + X^{(j)}_i }{n+1}\times\frac{S_y + k}{n+1}$$


==> Archive/otherfairness.tex <==
\section{Extension to Other Fairness Models}\label{sec:disc}
So far in this paper, 
we considered  independence ($\hat{y}\bot S$) for fairness.
Here we discuss how to extended our findings to other measures based on separation and sufficiency \cite{fairmlbook}, such as equalized odds \cite{hardt2016equality}, where the prediction outcome $\hat Y$ is independent of the sensitive feature $S$ given the true label $Y$, i.e. $P(\hat{y}=1|y = 1, S = 0)
= P(\hat{y}=1|y = 1, S = 1), y \in {0,1}$ 

% predictive parity, error rate balance, and accuracy equity~\cite{narayanan2018translation}.

FAL follows balancing fairness and misclassification error, using Equation~\ref{eq:opt}. Certainly, the entropy term $\mathcal{H}_{t-1}(y^{(i)})$ does not depend on the choice of fairness measure.
Also, the abstract fairness term $E\big[\mathcal{F}(C_{t}^i(.))\big]$ is not limited to a specific definition.
However, despite being abstract, computing the expected unfairness (based on separation or sufficiency) is challenging.

Looking at Figure~\ref{fig:EofF}, recall that we use the verification set $\mathcal{V}$ for estimating the fairness of a model.
As an unbiased sample set from $\mathcal{U}$, $\mathcal{V}$ follows the underlying data distribution and, hence, can be used for the demographic disparity.
However, this set cannot be used for estimating fairness according to separation or sufficiency since its instances are not labeled.
On the other hand, the pool of labeled data is not representative of the underlying data distribution.

We understand that since the labeling budget is limited, labeling $\mathcal{V}$ may reduce the number of instances we can use for training the model. One resolution is to limit $\mathcal{V}$ to a small set and accept the potential error in estimations.
In order to extend our results for other fairness measures, it is enough to label a random subset $\mathcal{C}_\mathcal{V}\subset\mathcal{V}$.
Once $\mathcal{C}$ is labeled, the equalized odds measure can be calculated, and our framework performs as-is for any such fairness measure using $\mathcal{C}$.
How small $\mathcal{V}$ can be to still provide accurate-enough estimations, besides other resolutions, are interesting questions that we will consider for future work.



==> Archive/plots-new.tex <==

\begin{figure*}[!t]
\centering     %%% not \center
\subfigure[]{\label{exp:base-compas}\includegraphics[width=0.32\linewidth]{figs/compas-all.pdf}}
\subfigure[]{\label{exp:base-adult}\includegraphics[width=0.32\linewidth]{figs/adult-all.pdf}}

\vspace{-3mm}
\caption{Comparison of baselines }\label{exp:base}
\end{figure*}

\begin{figure*}[!t]
\centering     %%% not \center
\subfigure[FAL $\alpha$-aggregate]{\label{exp:alpha-compas}\includegraphics[width=0.32\linewidth]{figs/alpha-compas.pdf}}
\subfigure[FAL Nested]{\label{exp:nested-compas}\includegraphics[width=0.32\linewidth]{figs/nested-compas.pdf}}
\subfigure[FAL Nested-Append]{\label{exp:append-compas}\includegraphics[width=0.32\linewidth]{figs/NAP-compas.pdf}}
\subfigure[FAL $\alpha$-aggregate \hadis{26 will update}]{\label{exp:alpha-adult}\includegraphics[width=0.32\linewidth]{figs/alpha-adult.pdf}}
\subfigure[FAL Nested]{\label{exp:nested-adult}\includegraphics[width=0.32\linewidth]{figs/nested-adult.pdf}}
\subfigure[FAL Nested-Append]{\label{exp:append-adult}\includegraphics[width=0.32\linewidth]{figs/NAP-adult.pdf}}
\vspace{-3mm}
\caption{The average DP and accuracy of different FAL approaches }\label{exp:fal}
\end{figure*}

\begin{figure*}[!t]
\centering     %%% not \center
\subfigure[FBC $\alpha$-aggregateL]{\label{exp:fbc-compas}\includegraphics[width=0.32\linewidth]{figs/fbc-alpha-compas.pdf}}
\subfigure[FBC Nested]{\label{exp:fbc-nested-compas}\includegraphics[width=0.32\linewidth]{figs/fbc-nested-compas.pdf}}
\subfigure[FBC Nested-Appen]{\label{exp:fbc-append-compas}\includegraphics[width=0.32\linewidth]{figs/fbc-nap-compas.pdf}}
\subfigure[FBC $\alpha$-aggregateL]{\label{exp:fbc-adult}\includegraphics[width=0.32\linewidth]{figs/fbc-alpha-adult.pdf}}
\subfigure[FBC Nested]{\label{exp:fbc-nested-adult}\includegraphics[width=0.32\linewidth]{figs/fbc-nested-adult.pdf}}
\subfigure[FBC Nested-Append]{\label{exp:fbc-append-adult}\includegraphics[width=0.32\linewidth]{figs/fbc-nap-adult.pdf}}
\vspace{-3mm}
\caption{The average DP and accuracy of different FBC approaches }\label{exp:fbc}
\end{figure*}

\begin{figure*}[!t]
\centering     %%% not \center
\subfigure[Accuracy]{\label{exp:acc-budget}\includegraphics[width=0.32\linewidth]{figs/acc-budget.pdf}}
\subfigure[Unfairness]{\label{exp:fair-budget-adult}\includegraphics[width=0.32\linewidth]{figs/fair-budget.pdf}}
\subfigure[Computation Time]{\label{exp:time}\includegraphics[width=0.32\linewidth]{figs/time.pdf}}
\vspace{-3mm}
\caption{--}\label{exp:budget}
\end{figure*}


\begin{figure*}[!t]
\centering     %%% not \center
\subfigure[Compas]{\label{exp:odds-compas}\includegraphics[width=0.32\linewidth]{figs/odds-compas2.pdf}}
\subfigure[Adult]{\label{exp:odds-adult}\includegraphics[width=0.32\linewidth]{figs/odds-adult.pdf}}
\vspace{-3mm}
\caption{Odds}\label{exp:odds}
\end{figure*}

==> Archive/plots.tex <==
% \begin{figure*}[ht]
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         \includegraphics[scale=0.32]{figures/FALvsAL_Mutinfo_flsk_compas.pdf}
%         \caption{Average DP (Mutual Information) of FAL vs. AL on Compas.}
%         \label{exp:FAL-demo}
%     \end{minipage}
%     \hfill 
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         \includegraphics[scale=0.32]{figures/FALvsAL_accuracy_flsk_compas.pdf}
%         \caption{Average accuracy score of FAL vs. AL on Compas.}
%         \label{exp:FAL-score}
%     \end{minipage}
%     \hfill
%         \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         \includegraphics[scale=0.32]{figures/FAL-adpative.pdf}
%         \caption{Accuracy vs. DP (Mutual Information) of FAL vs. AL and RandL on Compas. }
%         \label{exp:adaptive}
%     \end{minipage}
% \vspace{-3mm}
% \end{figure*}


\begin{figure}[!t]
\centering     %%% not \center
\subfigure[Unfairness]{\label{exp:FAL-demo}\includegraphics[scale=0.55]{figures/FALvsAL_Mutinfo_flsk_compas.pdf}}
\subfigure[Accuracy]{\label{exp:FAL-score}\includegraphics[scale=0.55]{figures/FALvsAL_Accur_flsk_compas.pdf}}
\subfigure[Accuracy vs. Unfairness]{\label{exp:adaptive}\includegraphics[scale=0.55]{figures/FAL-adpative.pdf}}
\caption{The average DP and accuracy of different methods on COMPAS.}\label{exp:fal-al}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.55]{figures/FAL-Adult.pdf}
    \caption{Accuracy vs. DP of FAL vs. AL and RandL on Adult.}
    \label{exp:adult}
\end{figure}
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.55]{figures/demoerr.pdf}
        \caption{Average DP (Absolute Difference) of FAL vs. AL on COMPAS.}
        \label{exp:demoerr}
\end{figure}
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.55]{figures/fml.pdf}
        \caption{Accuracy vs. DP, impact of FAL-FairLR on COMPAS.}
        \label{exp:fml}
\end{figure}

% \begin{figure*}[!t]
%     \begin{minipage}[t]{0.31\linewidth}
%         \centering
%         \includegraphics[scale=0.4]{figures/FAL-Adult.pdf}
%         \caption{Accuracy vs. DP of FAL vs. AL and RandL on Adult.}
%         \label{exp:adult}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.31\linewidth}
%         \centering
%         \includegraphics[scale=0.4]{figures/demoerr.pdf}
%         \caption{Average DP (Absolute Difference) of FAL vs. AL on COMPAS.}
%         \label{exp:demoerr}
%     \end{minipage}
%     \hfill 
%     \begin{minipage}[t]{0.31\linewidth}
%         \centering
%         \includegraphics[scale=0.4]{figures/fml.pdf}
%         \caption{Accuracy vs. DP, impact of FAL-FairLR on COMPAS.}
%         \label{exp:fml}
%     \end{minipage}
% \vspace{-3mm}
% \end{figure*}

% \begin{figure*}[ht]
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         \includegraphics[scale=0.32]{figures/fbc-fal-time.pdf}
%         \caption{FAL vs. FBC, time. }
%         \label{exp:time}
%     \end{minipage}
%     \hfill 
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         \includegraphics[scale=0.32]{figures/fal-fbc-demo.pdf}
%         \caption{FAL vs. FBC, fairness. }
%         \label{exp:fal-fbc-demo}
%     \end{minipage}
%         \hfill 
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         \includegraphics[scale=0.32]{figures/fal-fbc-score.pdf}
%         \caption{FAL vs. FBC accuracy }
%         \label{exp:fal-fbc-score}
%     \end{minipage}
% \vspace{-3mm}
% \end{figure*}


\begin{figure}[!t]
\centering     %%% not \center
\subfigure[Time]{\label{exp:time}\includegraphics[scale=0.55]{figures/fbc-fal-time.pdf}}
\subfigure[Unfairness]{\label{exp:fal-fbc-demo}\includegraphics[scale=0.55]{figures/fal-fbc-demo.pdf}}
\subfigure[Accuracy]{\label{exp:fal-fbc-score}\includegraphics[scale=0.55]{figures/fal-fbc-score.pdf}}
\vspace{-3mm}
\caption{Time, average DP, and accuracy of FAL vs. FBC on COMPAS.}\label{exp:fal-fbc}
%\vspace{-7mm}
\end{figure}


% % \begin{figure*}[ht]
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/accuracy-Cov.pdf}
% %     %     \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{12}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:accu12}
% %     % \end{minipage}
% %     % }
% %     % \hfill
% %     % {
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/cov-Cov.pdf}
% %     %     \vspace{-8mm}\caption{ $Fairness_{12}$ of FAL-$Fairness_{12}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:demo12}
% %     % \end{minipage}
% %     % }
% %     % \hfill
% %     % {
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/F1-Cov.pdf}
% %     %     \vspace{-8mm}\caption{F1-score of FAL-$Fairness_{12}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:f1_12}
% %     % \end{minipage}
% %     % }
% %     %     \hfill
% %     \begin{minipage}[t]{0.5\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/Cov-err.pdf}
% %         \vspace{-8mm}\caption{Accuracy versus $Fairness_{12}$. }
% %         \label{exp:demo12}
% %     \end{minipage}
% %         \hfill
% %     \begin{minipage}[t]{0.5\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/Cov-PR-err.pdf}
% %         \vspace{-8mm}\caption{Precision versus recall for $Fairness_{12}$. }
% %     % \hfill
% %     % \begin{minipage}[t]{0.5\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/precision-Cov.pdf}
% %     %     \vspace{-8mm}\caption{Precision/Recall of FAL-$Fairness_{12}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:pr12}
% %     \end{minipage}
% % \end{figure*}
% % \begin{figure*}[ht]
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/accuracy-demoErr.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{21}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:accu21}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoErr.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{21}$ of FAL-$Fairness_{21}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:demo21}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/F1-demoErr.pdf}
% %         \vspace{-8mm}\caption{F1-score of FAL-$Fairness_{21}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:f1_21}
% %     \end{minipage}
% %     }
% %         \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/precision-demoErr.pdf}
% %         \vspace{-8mm}\caption{Precision/Recall of FAL-$Fairness_{21}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:prec21}
% %     \end{minipage}
% %     }
% % \end{figure*}
% \begin{figure*}[ht]
%     % {
%     % \begin{minipage}[t]{0.2\linewidth}
%     %     \centering
%     %     \includegraphics[scale=0.3]{figures/accuracy-GErr.pdf}
%     %     \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{22}$ with different $\alpha$ values vs. AL and RL}
%     %     \label{exp:accu22}
%     % \end{minipage}
%     % }
%     % \hfill
%     % {
%     % \begin{minipage}[t]{0.2\linewidth}
%     %     \centering
%     %     \includegraphics[scale=0.3]{figures/GErr.pdf}
%     %     \vspace{-8mm}\caption{$Fairness_{22}$ of FAL-$Fairness_{22}$ with different $\alpha$ values vs. AL and RL}
%     %     \label{exp:demo22}
%     % \end{minipage}
%     % }
%     % \hfill
%     % {
%     % \begin{minipage}[t]{0.2\linewidth}
%     %     \centering
%     %     \includegraphics[scale=0.3]{figures/F1-GErr.pdf}
%     %     \vspace{-8mm}\caption{F1-score of FAL-$Fairness_{22}$ with different $\alpha$ values vs. AL and RL}
%     %     \label{exp:f1_22}
%     % \end{minipage}
%     % }
%     %     \hfill
%         \begin{minipage}[t]{0.208\linewidth}
%         \centering
%         \includegraphics[scale=0.3]{figures/GErr-err-1.pdf}
%         \vspace{-8mm}\caption{Accuracy versus $Fairness_{22}$. }
%         \label{exp:demo22}
%     \end{minipage}
%         \hfill
%     \begin{minipage}[t]{0.208\linewidth}
%         \centering
%         \includegraphics[scale=0.3]{figures/GErr-PR-err-1.pdf}
%         \vspace{-8mm}\caption{Precision versus recall for $Fairness_{22}$. }
%                 \label{exp:pr22}
%     \end{minipage}
%     \hfill
%       \begin{minipage}[t]{0.208\linewidth}
%         \centering
%         \includegraphics[scale=0.3]{figures/demoRatio-err-1.pdf}
%         \vspace{-8mm}\caption{Accuracy versus $Fairness_{31}$. }
%         \label{exp:demo31}
%     \end{minipage}
%         \hfill
%     \begin{minipage}[t]{0.208\linewidth}
%         \centering
%         \includegraphics[scale=0.3]{figures/demoRatio-PR-err-1.pdf}
%         \vspace{-8mm}\caption{Precision versus recall for $Fairness_{31}$. }
%                 \label{exp:pr31}
%     \end{minipage}
%     % {
%     % \begin{minipage}[t]{0.2\linewidth}
%     %     \centering
%     %     \includegraphics[scale=0.3]{figures/precision-GErr.pdf}
%     %     \vspace{-8mm}\caption{Precision/Recall of FAL-$Fairness_{22}$ with different $\alpha$ values vs. AL and RL}
%     %     \label{exp:prec22}
%     % \end{minipage}
%     % }
% \vspace{-4mm}
% \end{figure*}
% % \begin{figure*}[ht]
% %     % {
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/accuracy-demoRatio.pdf}
% %     %     \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{31}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:accu31}
% %     % \end{minipage}
% %     % }
% %     % \hfill
% %     % {
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/demoRatio.pdf}
% %     %     \vspace{-8mm}\caption{$Fairness_{31}$ of FAL-$Fairness_{31}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:demo31}
% %     % \end{minipage}
% %     % }
% %     % \hfill
% %     % {
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/F1-demoRatio.pdf}
% %     %     \vspace{-8mm}\caption{F1-score of FAL-$Fairness_{31}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:f1_31}
% %     % \end{minipage}
% %     % }
% %     %     \hfill
% %     % {
% %     % \begin{minipage}[t]{0.2\linewidth}
% %     %     \centering
% %     %     \includegraphics[scale=0.3]{figures/precision-demoRatio.pdf}
% %     %     \vspace{-8mm}\caption{Precision/Recall of FAL-$Fairness_{31}$ with different $\alpha$ values vs. AL and RL}
% %     %     \label{exp:prec31}
% %     % \end{minipage}
% %     % }
% %             \begin{minipage}[t]{0.5\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoRatio-err.pdf}
% %         \vspace{-8mm}\caption{Accuracy versus $Fairness_{31}$. }
% %         \label{exp:demo31}
% %     \end{minipage}
% %         \hfill
% %     \begin{minipage}[t]{0.5\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoRatio-PR-err.pdf}
% %         \vspace{-8mm}\caption{Precision versus recall for $Fairness_{31}$. }
% %                 \label{exp:pr31}
% %     \end{minipage}
% % \end{figure*}
% % \begin{figure*}[ht]
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/accuracy-GRatio.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{32}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:accu32}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/GRatio.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{32}$ of FAL-$Fairness_{32}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:demo32}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/F1-GRatio.pdf}
% %         \vspace{-8mm}\caption{F1-score of FAL-$Fairness_{32}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:f1_32}
% %     \end{minipage}
% %     }
% %         \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/precision-GRatio.pdf}
% %         \vspace{-8mm}\caption{Precision/Recall of FAL-$Fairness_{32}$ with different $\alpha$ values vs. AL and RL}
% %         \label{exp:prec32}
% %     \end{minipage}
% %     }
% % \end{figure*}
% % \begin{figure*}[ht]
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/MutInfo-accuracy-budget.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{11}$ vs. labeling budget}
% %         \label{exp:b:accu11}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/MutInfo-budget.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{11}$ of FAL-$Fairness_{11}$ vs. labeling budget}
% %         \label{exp:b:demo11}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/cov-accuracy-budget.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{12}$ vs. labeling budget}
% %         \label{exp:b:accu12}
% %     \end{minipage}
% %     }
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/cov-budget.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{12}$ of FAL-$Fairness_{12}$ vs. labeling budget}
% %         \label{exp:b:demo12}
% %     \end{minipage}
% %     }
% % \end{figure*}
% % \begin{figure*}[ht]
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoErr-accuracy-budget.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{21}$ vs. labeling budget}
% %         \label{exp:b:accu21}
% %     \end{minipage}
% %     }
% %         \hfill
% %     {
% %      \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoErr-budget.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{21}$ of FAL-$Fairness_{21}$ vs. labeling budget}
% %         \label{exp:b:demo21}
% %     \end{minipage}
% %     }  
% %     \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/GErr-accuracy-budget.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{22}$ vs. labeling budget}
% %         \label{exp:b:accu22}
% %     \end{minipage}
% %     }
% %         \hfill
% %     {
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/GErr-budget.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{22}$ of FAL-$Fairness_{22}$ vs. labeling budget}
% %         \label{exp:b:demo22}
% %     \end{minipage}
% %     }
% % \end{figure*}
% % \begin{figure*}
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoRatio-accuracy-budget.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{31}$ vs. labeling budget}
% %         \label{exp:b:accu31}
% %     \end{minipage}
% %         \hfill
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/demoRatio-budget.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{31}$ of FAL-$Fairness_{31}$ vs. labeling budget}
% %         \label{exp:b:demo31}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/GRatio-accuracy-budget.pdf}
% %         \vspace{-8mm}\caption{Accuracy score of FAL-$Fairness_{32}$ vs. labeling budget}
% %         \label{exp:b:accu32}
% %     \end{minipage}
% %         \hfill
% %     \begin{minipage}[t]{0.2\linewidth}
% %         \centering
% %         \includegraphics[scale=0.3]{figures/GRatio-budget.pdf}
% %         \vspace{-8mm}\caption{$Fairness_{32}$ of FAL-$Fairness_{32}$ vs. labeling budget}
% %         \label{exp:b:demo32}
% %     \end{minipage}
% % \end{figure*}

==> Archive/proofs.tex <==
\section{Proofs}

\stitle{Theorem~\ref{th:cov}:}
{\em
For a linear classifier in form of $\hat{y}=\theta^\top X$,
% Under the Assumption 1. 
$cov(S,\hat{y})=\theta^\top cov(S,X)$.
}
\begin{proof} 
% $cov(S,\hat{y})$ can be computed as $\theta^\top cov(S,X)$:
\begin{align*}
    cov(S,\hat{y})&=E[S\, \hat{y}] - E[S]E[\hat{y}]\\
    E[S]E[\hat{y}] &= \mu_S E\big[\sum\theta_ix_i\big] = \mu_S \sum\theta_i\mu_{x_i} \\
    &=\theta_1\mu_S\mu_{x_1}+\theta_2\mu_S\mu_{x_2}+\cdots+\theta_d\mu_S\mu_{x_d}\\
    E[S\hat{y}]&= E\big[S\,\sum\theta_ix_i\big] = E\big[\sum S\, \theta_ix_i\big]\\
    &=E\big[S\,\theta_1x_1+S\,\theta_2x_2+\cdots+ S\,\theta_d x_d \big]\\
    &=E\big[S\,\theta_1x_1\big]+E\big[S\,\theta_2x_2\big]+\cdots+ E\big[S\,\theta_d x_d \big]\\
    &=\theta_1E\big[S\,x_1\big]+\theta_2E\big[S\,x_2\big]+\cdots+ \theta_d E\big[S\, x_d \big]
\end{align*}

\begin{align}
    \nonumber \Rightarrow& cov(S,\hat{y})=\\ 
    \nonumber &\theta_1E\big[S\,x_1\big]+\theta_2E\big[S\,x_2\big]+\cdots+ \theta_d E\big[S\, x_d \big]\\
    \nonumber &- (\theta_1\mu_S\mu_{x_1}+\theta_2\mu_S\mu_{x_2}+\cdots+\theta_d\mu_S\mu_{x_d})\\
    \nonumber =&\theta_1(E\big[S\,x_1\big] - \mu_S\mu_{x_1})+\cdots+
    \theta_d(E\big[S\,x_d\big] - \mu_S\mu_{x_d})\\
    =&\sum\limits_{i=1}^d \theta_i cov(S,x_i) = \theta^\top cov(S,X)
\end{align}
\end{proof}

\stitle{Theorem~\ref{th:ALnotWork}:}
{\em
An active learning method with any sampling strategy that does not consider fairness may generate unfair models.
}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=.35\textwidth]{figures/proof.jpg}
    \vspace{-10mm}\caption{Illustration of proof by construction for Theorem~\ref{th:ALnotWork}.}
    \label{fig:proof-1}
\end{figure}
\begin{proof}
We provide the proof by construction.
In the following, we construct a case where between a pair of points, the one that worsens the fairness is preferred to be labeled.
Consider a toy 2D setting where $X=\{x_1, x_2\}$ are the features used for training a linear classifier $C(X) = \theta_1 x_1 + \theta_2 x_2$. Let {\tt \small color} be the binary sensitive attribute with values {\tt \small blue} and {\tt \small red}.
Assume the underlying distribution for the red points is uniform in range $[0,1]$ for $x_1$ and $x_2$ (the two features are independent for the red points).
Now consider an active learning method (AL) that has labeled a set of points $\mathcal{L}$, so far.
AL can use any arbitrary sampling strategy that is specified by a function $\mathcal{R}:\mathbb{R}^d\rightarrow \mathbb{R}^+$, which should get maximized, i.e., the points with higher scores are preferred.
Suppose using the labeled points $\mathcal{L}$, the current weights of the classifier are $\theta_1=1$ and $\theta_2=1$ and the decision boundary is at $x_1 + x_2 = 1$. That is, as shown in Figure~\ref{fig:proof-1} with the black solid line, for a point $P_i$, $\hat{y}^{(i)} = 1$ iff $x_1^{(i)}+x_2^{(i)}\geq 1$.

Now consider the two points $P_1$ and $P_2$ specified in the figure.
Note that AL chooses between $P_1$ and $P_2$ purely based on $X^{(1)}$ and $X^{(2)}$. That is, it prefers $\argmax(\mathcal{R}(X^{(1)}),\mathcal{R}(X^{(2)}))$ for choosing between these two points.
Suppose $P_1$ is the point that maximizes $\mathcal{R}$ and, hence, is preferred to be labeled next (the following argument can be easily adjusted if $P_2$ is preferred).
Suppose $y^{(1)}=1$ and $y^{(2)}=1$. Therefore, after labeling $P_1$ and adding it to $\mathcal{L}$, the decision boundary gets updated to $\ell_1$ (the dashed line in Figure~\ref{fig:proof-1}).
Suppose the dotted line $\ell_2$ would be the decision boundary if $P_2$ had been selected.

First, assuming that all lines $C(.)$, $\ell_1$, and $\ell_2$ divide the space by half, while considering the uniform distribution of red points in the space, for all three decision boundaries $\mathbb{P}(\hat{y}=1|${\tt\small color}$=${\tt\small red}$) = 0.5$.
Next, let the underlying distribution of blue points\footnote{Note that since AL does not consider demographic distributions for choosing the points, we have the freedom to pick the demographic distributions as we wish.} be
according to the blue ellipse in Figure~\ref{fig:proof-1} ($\ell_2$ and $\ell_2'$ are the eigen vectors of the covariance matrix of $x_1$ and $x_2$, while the eigen values are as specified by the intersection of blue ellipse with the two vectors).
In this setting, if $\ell_2$ was the decision boundary, $\mathbb{P}(\hat{y}=1|${\tt\small color}$=${\tt\small blue}$)$ would be $0.5$. However, since $P_1$ has been selected, $\ell_1$ is the decision boundary and, hence, $\mathbb{P}(\hat{y}=1|${\tt\small color}$=${\tt\small blue}$)>0.5$.
In other words, if AL had picked $P_2$ the model would satisfy demographic parity since $\mathbb{P}(\hat{y}=1|${\tt\small color}$=${\tt\small blue}$) = \mathbb{P}(\hat{y}=1|${\tt\small color}$=${\tt\small red}$) = 0.5$, but it picked $P_1$ that introduced demographic disparity.
\end{proof}


% \stitle{Theorem~\ref{th:convex}:}
% {\em
% The objective function in Equation~\ref{eq:opt2} is convex with respect to $x$ given any fairness measure listed in table~\ref{tab:DemoMeasures}.
% }

% \begin{proof} We prove this by construction. Assuming the given fairness measure is mutual information $I(\hat{y};S)$:
% \begin{align*}
%     &\alpha\, \mathcal{H}_{t-1}(y^{(i)}) + (1-\alpha)\big(1-E\big[\mathcal{F}(C_{t}^i(.))\big] \big)\\ 
%     &=-\alpha \sum_{k=1}^{K} \mathbb{P}(y=k|X, \mathcal{L})\log \mathbb{P}(y=k|X,\mathcal{L})\\
%     &+(1-\alpha) (1- \sum_{k=1}^{K} \mathcal{F}(\overline{C_k}(.)) \mathbb{P}(y=k|X^{(i)}))\\
%     &= -\alpha \sum_{k=1}^{K} \mathbb{P}(y=k|X, \mathcal{L})\log \mathbb{P}(y=k|X,\mathcal{L})+(1-\alpha) \\
%     &(1- \sum_{k=1}^K \mathbb{P}(y=k|X^{(i)}) \sum_{s\in S} \sum_{\hat{y}\in \{1,...,K\}} \mathbb{\bar P}(s,\hat{y}) \log\frac{\mathbb{\bar P}(s,\hat{y})}{\mathbb{\bar P}(s)\mathbb{\bar P}(\hat{y})})\\
%     &= -\alpha \sum_{k=1}^{K} \mathbb{P}(y=k|X, \mathcal{L})\log \mathbb{P}(y=k|X,\mathcal{L})+(1-\alpha) \\
%     &(1-\sum_{k=1}^K\mathbb{P}(y=k|X^{(i)})(\sum_{s\in S}\sum_{\hat{y}\in \{1,...,K\}} \mathbb{\bar P}(s)\mathbb{\bar P}(\hat{y}|s) \log \mathbb{\bar P}(\hat{y}|s)\\
%     &+\sum_{s\in S}\sum_{\hat{y}\in \{1,...,K\}} \mathbb{\bar P}(s|\hat{y}) \mathbb{\bar P}(\hat{y})\log \mathbb{\bar P}(\hat{y})))\\
%     &=-\alpha \sum_{k=1}^{K} \mathbb{P}(y=k|X, \mathcal{L})\log \mathbb{P}(y=k|X,\mathcal{L})+(1-\alpha)\\
% \end{align*}
% \begin{align*}
%     &(1-\sum_{k=1}^K \mathbb{P}(y=k|X^{(i)})\sum_{s\in S} \mathbb{\bar P}(s) \sum_{\hat{y}\in \{1,...,K\}} \mathbb{\bar P}(\hat{y}|s)) \log\mathbb{\bar P}(\hat{y}|s)\\ 
%     &-\sum_{k=1}^K \mathbb{P}(y=k|X^{(i)}) \sum_{\hat{y}\in \{1,...,K\}} \mathbb{\bar P}(\hat{y}) \log\mathbb{\bar P}(\hat{y})\sum_{s\in S} \mathbb{\bar P}(s|\hat{y}))\\
% \end{align*}
% Since the function $f(t)=t \log t$ is strictly convex for all positive $t$. In our proof we decomposed the objective function in Equation~\ref{eq:opt2}, to linear combinations of $t \log t$ functions. The linear combination of convex functions remains convex. Therefore, the objective function is convex and the convergence to a global optimum is guaranteed. The proof can be easily extend to any other fairness measures.
% \end{proof}

==> Archive/technical.tex <==
\section{Fair Active Learning (FAL)}\label{sec:alg}
%\vspace{-2mm}
\subsection{FAL $\alpha$-aggregate}\label{sec:objFunction}
%\vspace{-2mm}
By carefully selecting samples to label,
AL has the potential to mitigate algorithmic bias by incorporating the fairness measure into its sampling process.
Still, not considering fairness while building models can result in model unfairness.
As a na\"ive resolution, one could decide to drop the sensitive attribute from the training data.
This, however, is not sufficient since the bias in the features may cause model unfairness~\cite{buolamwini2018gender,zou2018ai,manrai2016genetic}.
%As we shall later show in Lemma~\ref{th:cov}, bias in labeled training data $\mathcal{L}$ is the reason for model unfairness.
%The samples selected for labeling in an active learning framework can significantly impact the fairness of a trained model.
Hence, a smart sampling strategy is needed to mitigate the bias.
%
\eat{
A question which might come to mind is that will any of the existing AL strategies generate fair models. The answer is: \textit{not necessarily}. We show this in Observation~\ref{th:ALnotWork}.
\begin{observation}\label{th:ALnotWork}
An active learning method with any sampling strategy that does not consider fairness may generate unfair models.
\end{observation}
Following Lemma~\ref{th:ALnotWork}, AL strategies that do not consider fairness may generate unfair models.
}
%
On the other hand, blindly optimizing for fairness could result in an inaccurate model.
%, the model may lose its purpose for accuracy while obtaining high performance is indeed the main objective in any ML framework, including active learning.
For instance, in Example~\ref{ex1}, consider a model that randomly classifies individuals as high-risk. This model indeed satisfies demographic parity since the probability of the outcome is (random and therefore) independent of $S$.
However, such a model provides zero information about how risky an individual is.

%We balance the fairness and accuracy trade-off
%by treating fairness as an intrinsic part of the AL sampling strategy.
%The goal is to minimize the misclassification error as well as unfairness (c.f. \S~\ref{sec:back-FM}).
%\techrep{ in order to develop fair classifiers for applications with limited labeled data, similar to Example~\ref{ex1} and Example~\ref{ex2}.}
Similar to AL, FAL is also an iterative process that selects a sample from the unlabeled pool $\mathcal{U}$ to be added to the labeled pool $\mathcal{L}$.
However, FAL considers both fairness and misclassification error as the optimization objective for the sampling step.
That is, to choose the next sample to be labeled, FAL selects the one that contributes the most to the reduction of the misclassification error as well as model unfairness.
Specifically, for a sample point $\langle X^{(i)},S^{(i)} \rangle\in\mathcal{U}$, we consider the Shannon entropy measure $\mathcal{H}_{t-1}(y^{(i)})$ for misclassification error, while considering demographic disparity $\mathcal{F}(C_{t}^i)$ for unfairness --- $C_{t}^i$ is the classifier trained on $\mathcal{L}$ at iteration $t$, after labeling the point $\langle X^{(i)},S^{(i)}\rangle$
and $\mathcal{H}_{t-1}(y^{(i)})$ is the entropy of the $y^{(i)}$ based on the current model $C_{t-1}$.
\eat{
One way of formulating the optimization problem for sampling is as following:
\vspace{-2mm}\begin{align}
\nonumber
\argmax_{\langle X^{(i)},S^{(i)}\rangle \in\mathcal{U}} ~~&~~ \mathcal{H}_{t-1}(y^{(i)})\\
\nonumber s.t.~~ & ~~\mathcal{F}(C_{t}^i) \leq \epsilon
\end{align}
where $\epsilon$ denotes the restriction imposed by some regulations for fairness consideration.
Similarly, one could consider misclassification error as a hard constraint while optimizing for fairness.
Both of these models can be reformulated as unconstrained optimizations
using \hadis{lagrangian has to be removed or clarified} Lagrange multipliers \cite{rockafellar1993lagrange}.
}
The formulation can be viewed as a multi-objective optimization for fairness and misclassification error.
Another perspective is to view the fairness as a regularization term to the optimization.
Equation~\ref{eq:opt} is consistent with both of these views and is therefore considered in our framework.
% (as in Equation~\ref{eq:opt}) using Lagrange multipliers \cite{rockafellar1993lagrange}.
\vspace{0mm}
\begin{align}
\label{eq:opt}
\argmax_{\langle X^{(i)},S^{(i)}\rangle \in\mathcal{U}}  \alpha\, \mathcal{H}_{t-1}(y^{(i)}) + (1-\alpha)\big(\mathcal{F}(C_{t-1})-\mathcal{F}(C_{t}^i)\big)
\end{align}
$(\mathcal{F}(C_{t-1})-\mathcal{F}(C_{t}^i))$ is the unfairness reduction (fairness improvement) term and the coefficient $\alpha\in[0,1]$ is the user-provided parameter that determines the trade-off between the model fairness and model performance. Values closer to $1$ put greater emphasize on model performance, while smaller values of $\alpha$ put greater importance on fairness.
%Our experimental results verify fairness improves substantially through FAL optimization while maintaining the accuracy level.
As we elaborate in \S~\ref{sec:exp}, entropy and fairness values are standardized to the same scale before being combined in Equation~\ref{eq:opt}.





%Having discussed the optimization function, next we will provide the details of our FAL framework.


% \vspace{-3mm}
\subsection{Framework}\label{sec:framework}
% \vspace{-2mm}
FAL is an iterative approach similar to standard active learning approaches.
As shown in Figure~\ref{fig:arch}, the central component of FAL is the sample selection unit (SSU) that chooses an unlabeled point $\langle X^{(i)},S^{(i)} \rangle$ from $\mathcal{U}$ and obtains the label from an oracle. The labeled point $\langle X^{(i)},S^{(i)},y^{(i)} \rangle$ is moved to $\mathcal{L}$, the set of labeled points.
The set of labeled points are used to train $C_t$, the classifier at iteration $t$.
In the next iteration, $t+1$, SSU employs $C_t$ and selects the next point to be labeled. This process continues until the budget for labeling is exhausted.


% \begin{figure}[!bt]
% \centering
% \includegraphics[width=0.4\textwidth]{figures/Arch.jpg}
% \caption{FAL framework.}
% \label{fig:arch}
% \end{figure}
%\begin{wrapfigure}{r}{0.3\textwidth}
\begin{figure}
\centering
    %\vspace{-3mm}
    \includegraphics[width=0.7\linewidth]{figures/Arch.jpg}
    %\vspace{-5mm}
    \caption{\small FAL framework.}
    \label{fig:arch}
    %\vspace{-2.5mm}
%\end{wrapfigure}
\end{figure}


%The sample selection unit is in charge of selecting the next point to be labeled.
Equation~\ref{eq:opt} is the basis for balancing the trade-off between fairness and misclassification error for the next sample selection.
A problem, however, is that at the time of evaluating the candidate points in $\mathcal{U}$, we still do not know their labels. However, to evaluate the impact of each point for fairness, we need to know what the model parameters will be after labeling and adding the point to $\mathcal{L}$.
This requires knowing {\em all} labels beforehand which contradicts with the fact that $\mathcal{U}$ is unlabeled.

\hadis{define t }

To resolve this issue, using a decision theoretic approach ~\cite{settles2009active}, we consider the \textit{expected unfairness reduction}: selecting the point that is expected to impart the largest reduction to the current model unfairness, \emph{after acquiring its label}. Therefore, instead of $\mathcal{F}(C_{t})$ in Equation~\ref{eq:opt}, we plug in the expected fairness $E\big[\mathcal{F}^{i}_{t}\big]$.  %, we use Equation~\ref{eq:opt2} to pick a sample. 
In this way, we are approximating the expected future fairness of a model using $\mathcal{L}\cup X, \forall X\in \mathcal{U}$ over all possible labels under the current model.
\eat{In other words, SSU should select the sample point  $X$, which if labeled and added to $\mathcal{L}$ would result in a new model with reduced unfairness.}
%
Consider a point $P_i\in\mathcal{U}$ and let
$C^{i,k}_t$ be the model after adding $P_i$ to $\mathcal{L}$ if its true label is $y^{(i)}=k$.
Of course, SSU does not know the label in advance. Hence, it must instead calculate the unfairness as an expectation over the possible labels.
% \vspace{-2mm}
% \begin{align}
% \label{eq:opt2}
% \argmax_{\langle X^{(i)},S^{(i)}\rangle \in\mathcal{U}} ~~ \alpha\, \mathcal{H}_{t-1}(y^{(i)}) + (1-\alpha)\big(\mathcal{F}(C_{t-1})-E\big[\mathcal{F}^{i}_{t}\big]\big)
% \end{align}
Equation~\ref{eq:E[f]} denotes the expected (un)fairness computation used by SSU:

\hadis{R: you cannot compute $P(y = k|X)$. Here you should say what you do use, you use the probability according to your model: $P(\hat{y} = k | X_i, X_L, Y_L).$
}

%\vspace{0mm}
\begin{align}
\label{eq:E[f]}
E\big[\mathcal{F}^{i}_{t}\big]  = \sum_{k=0}^{K-1} \mathcal{F}(C^{i,K-1}_t) \mathbb{P}(y=k|X^{(i)})
% \vspace{-6mm}
\end{align}



Using Figure~\ref{fig:EofF} for explanation, for every point $P_i=\langle X^{(i)},S^{(i)}\rangle$ in the unlabeled pool,
SSU considers different values of $\{0,\dots,K-1\}$ as possible labels for $P_i$.
For every possible label $y_k$, it updates the model parameters to the intermediate model $C^{i,k}_t$ using $\mathcal{L}\cup \{\langle X^{(i)},  S^{(i)}, k\rangle\}$.


%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}
\centering
    %\vspace{-3mm}
    \includegraphics[width=\linewidth]{figures/EXF.jpg}
    %\vspace{-5mm}
    \caption{\small Evaluation of a point $\langle X^{(i)},S^{(i)}\rangle\in\mathcal{U}$ for unfairness reduction.}
    \label{fig:EofF}
    %\vspace{-2.5mm}
\end{figure}
%\end{wrapfigure}



Since the points to be labeled are selective samples from $\mathcal{U}$, and moved from $\mathcal{U}$ to $\mathcal{L}$, after the process starts, neither $\mathcal{U}$ nor $\mathcal{L}$ can be seen as i.i.d. samples of the actual underlying distribution, and therefore, cannot be used to estimate the fairness.
However, $\mathcal{U}$ initially follows the underlying distribution.
Therefore, to create a dataset for evaluating the fairness of the model for sample selection, we utilized the initial unlabeled pool $\mathcal{U}$ and use in different FAL iterations.
%
Following the standard AL, at every iteration, for every possible label for a point $\langle X^{(i)},S^{(i)}\rangle$, SSU uses the current model $C_{t-1}$ for calculating $\mathbb{P}(y=k|X^{(i)})$.
\eat{Having the fairness measures and the probabilities for each possible outcome, the expected unfairness is computed by aggregating $\mathcal{F}(C^{i,k}_t) \mathbb{P}(y=k|X^{(i)})$ for different values of $k$ (Equation~\ref{eq:E[f]}).
After computing the expected unfairness for each data point in $\mathcal{U}$, SSU identifies the one that optimizes Equation~\ref{eq:opt2} and passes it to the labeling oracle.
}
Algorithm~\ref{alg:fal} shows the pseudo-code of FAL where Algorithm~\ref{alg:EofF} is invoked for computing the expected unfairness.
%\begin{wrapfigure}{L}{0.5\textwidth}
%\vspace{-3.5mm}
%    \begin{minipage}{0.5\textwidth}
      \begin{algorithm}[]
        \caption{Fair Active Learning}
        \begin{algorithmic}[1]
        \label{alg:fal}
        \small
        \FOR{$t=1$ to $B$}
            \STATE $max=0$
            \FOR{$i=1$ to $|\mathcal{U}|$}
                \STATE {\it H} =$-\sum_{k=0}^{K-1} \mathbb{P}(y=k|X)\log \mathbb{P}(y=k|X)$
                \STATE $F =$ {\bf ExpF}$\big(\langle X^{(i)},S^{(i)}\rangle,\mathcal{L},C_{t-1}\big)$
                \STATE $obj = \alpha(i) H + (1-\alpha(i))(\mathcal{F}(C_{t-1})-F)$
                \IF{$obj>max$}
                    \STATE $max = obj$;
                    $\langle X^*,S^*\rangle = \langle X^{(i)},S^{(i)}\rangle$
                \ENDIF
            \ENDFOR
            \STATE $y =$ label $X^*$ using the labeling oracle
            \STATE move $\langle X^*,S^*,y\rangle$ to $\mathcal{L}$
            \STATE train the classifier $C_t$ using $\mathcal{L}$
        \ENDFOR
        \STATE {\bf return} $C_t$
        \end{algorithmic}
      \end{algorithm}
 %   \end{minipage}
  %  \vspace{-5mm}
 % \end{wrapfigure}
 
% \begin{wrapfigure}{R}{0.45\textwidth}
% %\vspace{-4mm}
%     \begin{minipage}{0.45\textwidth}
       \begin{algorithm}[]
        \caption{{\bf ExpF}}
        \begin{algorithmic}[1]
        \label{alg:EofF}
        \small
        \REQUIRE $\langle X^{(i)},S^{(i)}\rangle,\mathcal{L},C_{t-1}$
        \STATE $sum=0$
        \FOR{$k=0$ to $K-1$}
            \STATE train $C^{i,k}_t$ using $\mathcal{L}\cup\{\langle X^{(i)},S^{(i)},y_k\rangle\}$
            \STATE compute $\mathcal{F}(C^{i,k}_t)$
            \STATE $sum = sum + \mathcal{F}(C^{i,k}_t) \mathbb{P}(y=k|X^{(i)})$
        \ENDFOR
        \STATE {\bf return} $sum$
        \end{algorithmic}
      \end{algorithm}
%     \end{minipage}
%   \end{wrapfigure}

% \subsection{Adaptive $\alpha$ parameter}\label{sec:adaptivealpha}

The trade-off between the accuracy (entropy) and the fairness terms is controlled by a user-defined parameter $\alpha$ (in Equation~\ref{eq:opt}).
Selecting an appropriate $\alpha$ value might not be clear for the user. More importantly, FAL might find it challenging to use a fixed learning strategy based on $\alpha$ in different iterations. \hadis{To avoid parameter tuning in active learning... we can summarize the following paragraphs without discussing the accuracy discussion}

In initial iterations, the model is not accurate because it was trained only on a few labeled instances, resulting in possibly inaccurate estimates of the label probabilities for a given unlabeled instance from $\mathcal{U}$.
Computing the expected fairness values relies heavily on the probabilities of the label. The miscalculation of these probabilities leads to an inaccurate estimation of fairness; such erroneous values contribute to the selection of points that do not support (and may even deteriorate) the fairness of the model and may not be good for model accuracy.
%Wrong samples selected due to the wrong estimation of unfairness may not be a good choice, either from accuracy nor fairness perspective.
In the later iterations, the model may already be stable and accurate, and new labeled points may not significantly impact its accuracy.
However, the model can provide better estimations of the label probabilities which results in more robust estimations of the expected fairness.
%The points that are introduced in the later iterations may not significantly impact the model accuracy, and yet can have a better impact on the model fairness improvement.

Instead of using a fixed $\alpha$ for all iterations, one can use a {\em decay function} that begins with a large value of $\alpha$, which improves the accuracy of the model. As the model becomes more stable, the value of $\alpha$ gets dropped, putting more weight on improving fairness.
This concept is applied in different context, such as assigning learning rate~\cite{schaul2013no}, where a larger value is used initially that gradually decreases over time.
Our approach is agnostic to the decay function used.
In the experiments, we use a function that linearly interpolates between a given range (such as [0.1, 0.9]).

\subsection{FAL Nested}\label{sec:topk}
Accurately estimating the expected unfairness reduction is critical for the performance of FAL.
Looking at Equation~\ref{eq:E[f]}, the value of expected fairness directly depends on the probability estimations of the current model $C_{t-1}$ for different class labels $k$.
Sacrificing accuracy for fairness in previous steps will affect the estimation of expected fairness in subsequent steps. Poor estimation of the expected unfairness improvement as a result, may mislead the sample selection to choose points that are not only not good for accuracy, but also not good for improving fairness.
In order to prevent this phenomena, it is necessary to always maintain an accurate intermediate model -- i.e., to ensure that the selected points to be labeled will not negatively impact the accuracy of the model.


Fortunately, we make an observation in practice that helps us keeping the intermediate models accurate while achieving fairness.
As we shall further explain in the following, our observation, also helps us to even reduce the computation cost of the model but only focusing on a subset of $\mathcal{U}$, instead of the full set.


It turns out in practice the distribution of the entropy of the data points in $\mathcal{U}$ is right-skewed, i.e. having a large number of points having entropy close to 1, i.e., all these points are almost equally good candidates from the accuracy perspective. We observed this in our real experiments, including the one on XXX dataset \abol{provide more details} -- shown in Figure~\ref{fig:edist}.

Consider the set of points on the right-most bucket with entropy close to one.
Any of the points in this set are good candidates from lens of active learning (Equation~\ref{eq:entropy}) to assure the high quality of the intermediate models.
On the other hand, the relatively large size of the set (as observed in Figure~\ref{fig:edist}) gives us the opportunity to select the point with highest potential for reducing unfairness.






\begin{figure}
\centering
    %\vspace{-3mm}
    \includegraphics[width=\linewidth]{figures/e_distn.pdf}
    \vspace{-7mm}
    \caption{\small Distribution of Entropy for Compas dataset.}
    \label{fig:edist}
    \vspace{-5mm}
%\end{wrapfigure}
\end{figure}

% \begin{figure}
% \centering
%     %\vspace{-3mm}
%     \includegraphics[width=0.7\linewidth]{figures/distn_grid.pdf}
%     %\vspace{-5mm}
%     \caption{\small Distribution}
%     \label{fig:dist}
%     \vspace{-5mm}
% %\end{wrapfigure}
% \end{figure}
\eat{
Note that the points with largest entropy may not be the same points with largest unfairness reduction. Hence, when we combine the entropy and fairness metric with the control parameter $\alpha$, the distribution of the score based on Equation~\ref{eq:opt} will be less skewed as we decrease $\alpha$. This allows SSU selects the points that are not improving the accuracy necessarily (the points that does not belong the largest bucket on $\mathcal{H}$ distribution). We would like to underscore that the high accuracy of the model after adding the selected candidate point is critical to accurately estimating the expected (un)fairness reduction values in the subsequent iterations. 
Hence, sample selection based on the combined score, Equation~\ref{eq:opt}, in such situation may result in a less accurate model, and misleading the SSU in choosing the points that will improve the (un)fairness reduction. 
In this section, we propose a hierarchical sampling for accuracy-fairness trade-off to address this issue and prevent the random selection. 
}

We use the above observation to design a {\em nested optimization} for accuracy and fairness. 
In particular, instead of computing a score by linearly combining the two terms (Equation~\ref{eq:opt}), we apply a two-level optimization where in the first level, we select a subset of $\mathcal{U}_A \subset \mathcal{U}$ of the top-$\ell$ points\footnote{Instead of a fixed set cardinality, one could consider selecting the points that their values are close to the maximum (e.g. have distance less than 0.001).} that maximize the entropy $\mathcal{H}(y^{(i)})$ using the current classifier $C_{t-1}$:

\begin{align*}
    \mathcal{U}_A = \underset{\langle X^{(i)},S^{(i)}\rangle \in\mathcal{U}}{\ell\mbox{-argmax}} \mathcal{H}(y|X,\mathcal{L})
\end{align*}

where the function $\ell$-argmax returns $\ell$ samples with maximum values.
The first optimization level only optimizes for accuracy, to assure maintaining a high accuracy for the intermediate model.
The next level optimization 
Next, changing the optimization criteria to fairness in the second level, SSU selects a point from $\mathcal{U}_A$ that maximizes the unfairness improvement (Equation~\ref{eq:top-kp2}) and pass it to the labeling oracle. 
\begin{align}
    \nonumber&\argmax_{\langle X^{(i)},S^{(i)}\rangle \in\mathcal{U}_A} \big(\mathcal{F}(C_{t-1})-\mathcal{F}(C_{t}^i)\big)\\
    =& \argmin_{\langle X^{(i)},S^{(i)}\rangle \in\mathcal{U}_A} \mathcal{F}(C_{t}^i)
    \label{eq:top-kp2}
\end{align}


\eat{
Consider $\mathcal{U}_A\subset \mathcal{U}$ a set of cardinality $\ell$ maximizing entropy $\mathcal{H}(y^{(i)})$ using the current classifier $C_{t-1}$. $\forall P_i \in \mathcal{U}_A$ we evaluate the expected (un)fairness reduction $E\big[\mathcal{F}^{i}_{t}\big]$. The points with the maximum $E\big[\mathcal{F}^{i}_{t}\big]$ value will be selected to be labeled next. When $\ell=1$ FAL top-$\ell$ performs similar to active learning itself. The smaller the $\ell$ is the more weight the SSU puts on accuracy.
As $\ell$ increases SSU will have access to more points that improves the expected unfairness reduction. 
}

Besides assuring the accurate estimations of expected unfairness reduction, the two-level optimization helps to reduce the time-complexity of FAL.
This is in particular important as it reduces the number of points to be evaluated for fairness from $|\mathcal{U}|$ to $\ell$.
Note that, in order to estimate the unfairness reduction for every sample (Figure~\ref{fig:dist}), FAL requires to retrain $k$ models. As a result, the computation time to run the framework is dominated by the total time to compute fairness values for the points in the unlabeled pool, before selecting one to be labeled.
As a result, reducing the number of points to be evaluated for fairness significantly reduces the computation cost by a factor of $\frac{\ell}{|\mathcal{U}|}$.


% It is worth noting that the computation time of FAL top-$\ell$ approach significantly improves compare to FAL since we the expected (un)fairness reduction is only evaluated for the restricted dataset $\mathcal{U}_{|A|}$ with size $\ell$.

\subsection{FAL Nested Append}
Although in FAL Top-$\ell$ approach SSU selects points with maximum expected (un)fairness reduction from the top-$\ell$ maximum entropy points, the selected candidate might not necessarily improve the true (un)fairness reduction due to the low overall accuracy of the current classifier (especially in the initial iterations). To further improve the true (un)fairness level of the classifier, we propose to replicate the points that actually improve the true (un)fairness reduction after it is labeled. In this way we assign a weight to every point according to its contribution to the true (un)fairness reduction. 

Let $\Tilde{P}_i=\langle \Tilde{X}^{(i)},\Tilde{S}^{(i)}\rangle \in \mathcal{U}_A$ be the selected point using FAL top-$\ell$ approach. After collecting the true label for $\Tilde{P}_i$, let $\Tilde{C}^{i,k}_t$ be the model and $\Tilde{\mathcal{F}}^{i}_{t}$ be the true (un)fairness of the model after adding $\Tilde{P}_i$ to $\mathcal{L}$ if its true label is $\Tilde{y}^{(i)}=k$. $\langle \Tilde{X}^{(i)},\Tilde{S}^{(i)}\rangle,k$ will be replicated once if $\mathcal{F}^{i}_{t-1}-\Tilde{\mathcal{F}}^{i}_{t} > 0$.

\begin{figure}
\centering
    %\vspace{-3mm}
    \includegraphics[width=0.7\linewidth]{figures/append.pdf}
    %\vspace{-5mm}
    \caption{\small Distribution of Entropy for Compas dataset.}
    \label{fig:append}
    \vspace{-5mm}
%\end{wrapfigure}
\end{figure}









% \abol{if we have space, we can discuss the (easy) extension to multiple sensitive attributes in the discussions section}
% \textcolor{blue}{May be add it here?}

